Individual Fairness in Graph Decomposition

In this paper, we consider classic randomized low diameter decomposition procedures for planar graphs that obtain connected clusters which are cohesive in that close-by pairs of nodes are assigned to the same cluster with high probability. We require the additional aspect of individual fairness - pairs of nodes at comparable distances should be separated with comparable probability. We show that classic decomposition procedures do not satisfy this property. We present novel algorithms that achieve various trade-offs between this property and additional desiderata of connectivity of the clusters and optimality in the number of clusters. We show that our individual fairness bounds may be difficult to improve by tying the improvement to resolving a major open question in metric embeddings. We finally show the efficacy of our algorithms on real planar networks modeling congressional redistricting.

==> content/extra.tex <==
\subsection{Random Weights}\label{sec:rand-wts}
\begin{algorithm}
	\caption{Klein-Plotkin-Rao with random weights}\label{alg:kpr-randwts}
	\hspace*{\algorithmicindent} \textbf{Input}: Integer $R$, planar graph $G=(V,E)$
	\begin{algorithmic}[1]
		\State Set $F\gets \{\}$.
		\For{$i=\{1,2,3\}$}
			\For{every connected component $C$
			of $G\setminus F$}
			\State Perform BFS from an arbitrary root $r$ in $C$.
			\State Sample $k$ uniformly at
			random from $\{0,1,\ldots R-1\}$.
			\For{every vertex $v$ at level $\ell\equiv k\mod R$}
			\State Choose $b\in \{0,1\}$ uniformly at random.
			\If{$b=0$}
			\State Let $E_v$ be the set of edges
			from $v$ to vertices in levels $\ell-1$
			and $\ell$.
			\gov{This is not right. I am thinking of another way to phrase this without making it overly complicated.}
			\ElsIf{$b=1$}
			\State Let $E_v$ be the set of edges
			from $v$ to vertices in level $\ell+1$.
			\EndIf
			\State $F\gets F\cup E_v$.
			\EndFor
			\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}

\begin{theorem}
	\Cref{alg:kpr-randwts}
	produces components of diameter $O(R)$
	and for every $u,v\in V(G)$, satisfies
	\begin{align*}
		\frac{1}{2R}\leq \Pr[u,v \text{ are separated}]\leq \frac{3(d(u,v)+1)}{R}.
	\end{align*}
\end{theorem}
\begin{proof}
	The diameter guarantee follows from the proof of
	\cref{lem:KPR}. Each phase effectively has at most
	$R+1$ levels of the BFS tree, and we can use the bounds from running KPR with parameter $R+1$.
	
	To get the upper bound on the separation probability, we only note the vertices of the shortest path between $u,v$ span $\leq d(u,v)+1$
	levels of the BFS Tree. With probability $1-\frac{d(u,v)+1}{R}$, none of these levels $\ell$	satisfy $\ell \equiv k\mod R$.
	Since there are 3 phases, a union bound 
	gives us the required bound.
	
	To get the lower bound on the probability of
	separation, consider the first phase.
	Assume without loss of generality that
	$u$ is at least as high as $v$ in the BFS Tree.
	If $u$ and $v$ are at the same level $\ell$,
	then with probability $\frac{1}{R}$,
	$k$ is chosen as $\ell \mod R$.
	It is easy to see that with probability $\frac{1}{2}$, $u$ and $v$
	are separated from each other.
	\gov{Elaborate.}
		
\end{proof}


\subsection{Extension to the Euclidean Plane and Non-Planar Graphs}
\km{Can we omit this section unless you are saying something concerte? Right now, it seems like a collection of trivial observations. Maybe mention something in the conclusion. Maybe just say that our results except Theorem 1.5 extend as is to $K_{r,r}$? }

Our results leverage the KPR framework and naturally extend to graphs
that exclude a $K_{r,r}$
minor. This results in a gradual
deterioration of our bounds
with the progressive inclusion of $r$ factors in the bounds.

Regarding the Euclidean plane, we have two cases. If we are dealing with points in $\mathbb{R}^2$,
then there is no direct analogue to (CON). In the
absence of (CON), existing methods
such as random projections
and random grids give us
almost-optimal results
for (COMP) and (CUT).
If instead, the input consists of a partition
\margingov{except for the boundaries? I need to make this a bit more formal.}
of some compact
space of $\mathbb{R}^2$,
then there is a straightforward analogue of (CON).
We could define a cluster to be connected if it
consists of compact sets whose union is also compact.
The adjacency relation in this
setting precisely
corresponds to a planar graph.

\gov{Is it okay to just talk about the plane?}




\iffalse



\begin{table}[tb]
	\centering
	\begin{tabular}{@{}ccc@{}}
		\toprule
		State & \cref{alg:kpr} & \cref{alg:kpr-randwts} \\ \midrule
	North Carolina	& 0.75 & 0.38\\ \midrule
 	Maryland	 & 0.78 & 0.42\\ \midrule
  Pennsylvania	 & 0.80 & 0.45\\
 \bottomrule
	\end{tabular}
	\caption{Average of Spearman's rank correlation coefficient $\psi$ for different states.
    The standard deviation was smaller than 0.03 for all experiments.}
	\label{tab:my-table2}
\end{table}


\gov{Need to work more on this.}
\paragraph{Individual Fairness.}
We find that \cref{alg:kpr-randwts}
is fairer from the 
perspective of edge separation
probabilities, as compared to \cref{alg:kpr}.

Since the graphs contain many
thousands of edges, we analyze this
property collectively. We do this in the following way: Consider 100 different runs of the algorithm (\cref{alg:kpr} or \cref{alg:kpr-randwts}).
Make a ranking of the edges based on how many of the runs separated the edge.
 Repeat this 21 times to get 21 such rankings of the edge.
 Let $\mathcal{R}_0$
    be the first ranking.
    Find the Spearman's rank correlation coefficient $\psi$
    between $\mathcal{R}_0$
    and each of the other
    rankings.

We find that $\psi$ is 
always much higher for \cref{alg:kpr}
than for \cref{alg:kpr-randwts}.
We report the results
in \cref{tab:my-table2}.


\fi


\iffalse

\gov{My opinion is that we skip this section entirely. I feel that the results don't look great for our worst state (NC) on paper. A valid criticism is that if you have one cluster with 50\% of the ideal population already, it may be very difficult to draw a district with it.
Our redistricting experiments show that this is not the case, and even with such large clusters, there are usually enough small clusters around them that we can make a good plan.

Since we are leaving out the redistricting plans, we lose this nuance and it seems worse than it is.
}


\paragraph{Population Balance.}
Though the population of the largest cluster may be large,
in practice we find that we
are still able to find clusterings
with deviation only 10\% from
optimal.

% \begin{figure}[htbp]
% \centering
% \begin{subfigure}[b]{0.49\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{expimg/plot_popMD.png}
%     \caption{Maryland.}
% \end{subfigure}
% \begin{subfigure}[b]{0.49\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{expimg/plot_popNC.png}
%     \caption{North Carolina.}
% \end{subfigure}
% \caption{Histogram of population of clusters for two states across 200 runs. The x-axis represents the population as a proportion of the ideal population.}
% \end{figure}


\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\linewidth]{expimg/plot_max_popNC.png}
\caption{Histogram of population of clusters for North Carolina across 200 runs. The x-axis represents the population as a proportion of the ideal population.}
\end{figure}

\fi

==> content/junk.tex <==


We assume for the sake of contradiction that $u,v$ are not separated with probability $\left(\frac{\rho_{uv}}{100}\right)^4$. Then we consider one run of the algorithm where they belonged to the same connected component in Step~\ref{alg2-step:phase} for both $i = 1,2$. Let these connected components be $G_1,G_2$. Suppose the chosen roots for $G_1, G_2$ in the corresponding iteration was $r_1,r_2$, and let the corresponding BFS trees be $T_1,T_2$ respectively.  Let $d_i(x,y)$ denote the distance between $x,y$ in $G_i$ for $i \in \{1,2\}$. We use the shorthand $\ell_i(u)$ for $d_i(r_i,u)$, that is the level of the tree $T_i$ (measured from the root) that $u$ belongs to.
	
We now define the random event. Recall that for every $R$ levels of the tree, we make two cuts in each iteration of Step~\ref{alg2-step:phase}. The event is related to where these cuts are made.

\begin{definition}[Sandwich Event]
For $i \in \{1,2\}$, we call a `sandwich event' in $T_i$ the event where the random numbers chosen in Step~\ref{alg2-step:sample-k1k2} satisfy
    \begin{itemize}
\item $k_1\equiv \ell \mod R$ for some $\ell$ satisfying 
$$\min (\ell_i(u),\ell_i(v))\geq \ell \geq \min(\ell_i(u),\ell_i(v))-\frac{d}{100}$$
\item $k_2\equiv \ell \mod R$ for some $\ell$ satisfying 
$$\max (\ell_i(u),\ell_i(v))\leq \ell \leq \max(\ell_i(u),\ell_i(v))+\frac{d}{100}$$
\end{itemize}	
	\end{definition}



Conditio

\km{What if the level corresponding to $\ell$ does not exist? Is the probability lower bound still valid?}
 
In other words, the sandwich event happens when the first cut (corresponding to $k_1$) for that iteration $i$ is made within $\frac{d}{100}$	levels above the higher of the levels of $u,v$ in $T_i$ and the second cut (corresponding to $k_2$) in that iteration is made within $\frac{d}{100}$ levels below  the level of the lower of $u,v$ in $T_i$. Observe that for a sandwich event to happen, $k_1$ and $k_2$ must each take one of $\frac{d}{100}$ possible values, this happens with probability $\left(\frac{d}{100R}\right)^2=\left(\frac{\rho_{uv}}{100}\right)^2$.

Let $E_1,E_2$ be the events that a sandwich event occurs in $T_1$ and $T_2$ respectively. Let $L_1$ be the event that $\abs{\ell_1(u)-\ell_1(v)}<\frac{d}{100}$. 

\km{Where does $\rho^2$ come from in the proof below?  }

\begin{claim}\label{claim:gap-small-g1}
$\Pr[L_1]\geq 1-\frac{\rho_{uv}}{100}$.
\end{claim}
\begin{proof}
If the event $\overline{L_1}$ occurs, that is, $\abs{\ell_1(u)-\ell_1(v)}\geq \frac{d}{100}$, then $u,v$ are split with probability at least $\frac{\rho_{uv}}{100}$. Thus, if the claim was not true, we get
$\Pr[u,v \text{ are separated}]\geq \left(\frac{\rho_{uv}}{100}\right)^2$ which contradicts our initial assumption that $u,v$ are not separated with probability $\left(\frac{\rho_{uv}}{100}\right)^4$.
\end{proof}

\km{Why is $E_1$ independent of $L_1$? It's not obvious for the way $k_1, k_2$ are chosen. Maybe simply argue that $\Pr[E_1 | L_1]$ is the correct value? }
 
We now condition on the events $L_1$ and $E_1$. These two events are independent by definition. From \cref{claim:gap-small-g1}
	and our earlier observation about $\Pr[E_1]$, we get
	$\Pr[L_1\cap E_1]\geq \left(\frac{\rho_{uv}}{100}\right)^2(1-\frac{\rho_{uv}}{100})\geq \frac{1}{4}\left(\frac{\rho_{uv}}{100}\right)^2$ noting that $\rho_{uv}\leq 1$.
	Let $L_2$ be the event that $\abs{\ell_2(u)-\ell_2(v)}<\frac{d}{100}$.
	\begin{claim}\label{claim:gap-small-g2}
	$\Pr[L_2|E_1\cap L_1]\geq 1- \frac{\rho_{uv}}{100}$.
	\end{claim}
	\begin{proof}
		If the event $\overline{L_2}$ occurs, that is, $\abs{\ell_1(u)-\ell_1(v)}\geq \frac{d}{100}$, then $u,v$ are again split with probability
		at least $\frac{\rho_{uv}}{100}$.
		We know that $\Pr[L_1\cap E_1]\geq \frac{1}{2}\left(\frac{\rho_{uv}}{100}\right)^2$.
		If the claim were not true,
		then this gives us
		$\Pr[u,v \text{ are separated}]\geq \frac{1}{4}\left(\frac{\rho_{uv}}{100}\right)^3$
		which again contradicts our initial assumption
	\end{proof}

\km{Again, I don't see the independence.}

The event we will study is  $L_1\cap L_2\cap E_1\cap E_2$.
	Note that $E_2$ is 
	independent of $L_1,L_2$ and $E_1$
	by definition.
	Thus we have
	$$\Pr[L_1\cap L_2\cap E_1\cap E_2]=\Pr[E_2]\cdot \Pr[L_2|E_1\cap L_1] \cdot \Pr[E_1\cap L_1]\geq \frac{1}{16}\left(\frac{\rho_{uv}}{100}\right)^4$$
	which is the LHS of the equation
	in \cref{thm:kpr-2cuts}.
	\Cref{lem:kpr-2cuts-main}
	then completes the proof of \cref{thm:kpr-2cuts}.





 For points $u,v$, let $d(u,v)$ be their
distance in the original planar graph and let
$d'(u,v)$ be their distance in the Euclidean
metric.
Let $\vec{x}$ be the random unit vector.
Then the probability that they are split is
\begin{align*}
	\Pr[u,v \text{ are separated by a hyperplane}] &=
	\int \Pr[\abs{(\vec{u}-\vec{v})\cdot \vec{x}}=i ]\frac{i}{R}di\\
	&=\frac{\mathbb{E}[\abs{(\vec{u}-\vec{v})\cdot \vec{x}}]}{R}\\
	\intertext{Because the projection of $\vec{u}-\vec{v}$  along a random vector unit vector in $D$ dimensions is approximately $\frac{\norm{\vec{u}-\vec{v}}}{\sqrt{D}}$,}
	\Pr[u,v \text{ are separated by a hyperplane}]&\approx \frac{d'(u,v)}{R \sqrt{\log n}} 
\end{align*}
Thus, we have
\begin{align*}
	\Pr[u,v \text{ are separated by a hyperplane}]&\geq  \frac{d(u,v)}{R \sqrt{\log n}}\\ 
	\Pr[u,v \text{ are separated by a hyperplane}]&\leq  \frac{d(u,v)}{R } 
\end{align*}






\paragraph{Embedding implies LDD}

\km{This direction is not interesting if it only holds for fixed $R$.}

Given a graph $G$, let $d(u,v)$ denote
the shortest path between $u,v$ in the graph $G$.
Suppose there is a non-contractive embedding into $\ell_1^{k}$ of distortion $w$, for some finite $k$. Let $f:V(G)\to \mathbb{R}^k$ denote the embedding function
and let $f_i(v)$ denote the $i^{th}$ coordinate of $f(v)$. For every $u,v\in V(G)$, we have
\[
d(u,v) \leq \mathbb{E}[\norm{f(u)-f(v)}_1] \leq w d(u,v)
\]

We argue that there is an LDD procedure for any parameter $R\geq w k \Delta$ where $\Delta$ is the diameter of the graph. We describe the process: Choose a coordinate $i$ uniformly at random.
Sample $\theta \in [0,\frac{R}{k})$ uniformly at random.
A vertex $v$ is in cluster $\delta$ if $f_i(v)\in \left[\frac{\delta R}{k}+\theta, \frac{(\delta+1)R}{k} +\theta \right]$.

Conditioned on the $i^{th}$ coordinate being chosen, the probability that $u,v$ are separated is exactly $$\min\left(\frac{k\abs{f_i(u)-f_i(v)}}{R},1\right)=\frac{k\abs{f_i(u)-f_i(v)}}{R}$$
for large $R$... Figure out the full argument.
\gov{Finish the argument.}


%\begin{claim}\label{claim:w-exists}
%There exists a vertex $w\in P$ .such that $d_2(u,w)\geq \frac{d}{2}-1$ and $d_2(v,w)\geq \frac{d}{2}-1$
%\end{claim}
%\begin{proof}
%Let $P$ have $p+1$ vertices. Index the vertices in $P$ starting from $u$ as $x_1,\ldots,x_{p+1}$. Observe that the second vertex satisfies $d_2(x_2,u)=1$ and the penultimate vertex satisfies $d_2(x_p,u)\geq d-1$, since $d_2(u,v)\geq d$. Furthermore, since $d_2(x_i,u)$ changes from $d_2(x_{i-1},u)$ by at most one, there must be some vertex $x\in P$ such that $d_2(x,u)=\frac{d}{2}-1$. Since $d_2(u,v)\leq d_2(x,u)+d_2(x,v)$, we get $d_2(x,v)\geq \frac{d}{2}-1$.
%\end{proof}

==> content/narrative.tex <==




%\section{A Sampling Scheme with Provable Guarantees}
%\km{The framework needs a name. How about {\sc LDDist}?}

%In this paper, we consider the question of efficiently generating random feasible plans (with running time comparable to ReCom) with some basic provable guarantees on the distribution over plans and on the compactness of the plans thus generated. Our framework uses random graph decompositions instead of Markov chains, and has two steps. 

\section{Low Diameter Decomposition and Fair Partitioning}
\label{sec:ldd}
As a first step, we choose a parameter $R$ and perform an LDD of $G$. We define an LDD below. 

\begin{definition} [Low Diameter Decomposition]
\label{def:ldd}
Given a graph $G(V,E)$ with shortest path distance $d(\cdot, \cdot)$, and given a parameter $R$, a low-diameter decomposition (LDD) is a (possibly randomized) partition of $V$ into disjoint clusters $\pi_1, \pi_2, \ldots, \pi_r$, so that for $j$ and $u,v \in \pi_j$, $d(u,v) = O(R)$.
\end{definition}

We first present the procedure of Klein, Plotkin, and Rao~\cite{KPR} in \cref{sec:kpr} that performs an LDD of a planar graph. We describe our modification to incorporate individual fairness in \cref{sec:improve}, and describe the theoretical tradeoffs between individual fairness and the desiderata of connectivity and compression in the LDD in \cref{sec:theory-intro}. We finally describe how to implement this step and the empirical observations about LDDs in \cref{sec:implement1}. %  Such a procedure guarantees that pairs of vertices $(u,v) \in V \times V$ with graph distance $d(u,v)$ are separated with probability at most a constant factor of the natural baseline, $\rho_{uv} = \frac{d(u,v)}{R}$. This is classically termed {\em low diameter decomposition} (LDD), and can be viewed as a guarantee on the distribution over plans via its {\em marginal} on vertex pairs. Such a guarantee on the marginal follows for planar graphs from the celebrated result of Klein, Plotkin, and Rao (KPR)~\cite{KPR}, who compute a randomized partition into connected regions of diameter at most $R$, for any parameter $R$. 




\subsection{Improved LDD via Individual Fairness}
\label{sec:improve}
When considering low diameter decompositions for the redistricting application, there are three desiderata that such a scheme should satisfy: 

\begin{enumerate}
\item Each part in the decomposition should be connected, with diameter $O(R)$. \cref{alg:kpr} guarantees this.
\item If we replace each part by a super-node, the number of super-nodes should be much smaller than $n = |V|$ regardless of the outcome of the randomness.  This condition captures that that the LDD compresses the graph, and will be required to ensure that Step (2) of the redistricting process that we outline later is computationally efficient.  This compression condition is difficult to formally reason about in general planar graphs. However, \cref{alg:kpr} ensures that for a path graph with $n$ nodes, the path is split into $O(n/R)$ components, which is the best possible compression.


\item Since our ultimate goal is to generate a close to uniform distribution over feasible partitions, the LDD should ideally spread the probability mass evenly across different decompositions. In terms of marginals, this translates to saying that for different pairs $(u,v)$ of vertices with comparable $d(u,v)$, the probability of separation should be comparable to $\rho_{uv}$. This is  analogous to notions of {\em individual fairness} that have been widely considered in machine learning literature~\cite{DworkIndividual}. The question we ask for LDDs is: {\em Can this property be achieved? } 
\end{enumerate}

To understand the final question about individual fairness better, consider the following example, where for different pairs $(u,v)$ whose $d(u,v)$ are comparable, the separation probability is indeed $\Theta(\rho_{uv})$ and hence comparable. In other words, the partitioning scheme treats different such pairs fairly in terms of separation probability.

\begin{example}
\label{eg:grid}
Consider a grid graph, where each vertex $v$ with coordinates $(i,j)$ has edges to the vertices with coordinates $(i-1,j)$, $(i+1,j)$, $(i,j-1)$, and $(i,j+1)$. A simple LDD is to choose $(\ell,m)$ uniformly at random from $[R] \times [R]$ and cut along the $x$-axis at $\{\ldots, \ell - 2R, \ell -R,  \ell, \ell + R, \ldots \}$ and the $y$-axis at $\{\ldots, m - 2R, m -R,  m, m + R, \ldots \}$. Then the probability any pair of vertices $(u,v)$ is separated is at least $\frac{\rho_{uv}}{2}$ and at most $\rho_{uv}$. 
\end{example}

\paragraph{An Impossibility Result.} The above example may give us hope that \cref{alg:kpr} also  recreates such an individual fairness guarantee for general planar graphs. Note that \cref{lem:KPR} implies an upper bound of $O(\rho_{uv})$ on the probability any pair $(u,v)$ of vertices is separated, but no corresponding lower bound.  

Our first result states, somewhat counter-intuitively, that \cref{alg:kpr} {\em does not} provide such a lower bound -- different vertex pairs of comparable distance can be separated with vastly different probabilities, and this holds even when the vertex pair is an edge. 

\begin{theorem}[Proved in \cref{sec:kpr-negative}]
\label{thm:kpr-negative}
For any $n\in \mathbb{N}$ and $1\leq d\leq \frac{\sqrt{n}}{3}$, there exists a planar graph $G_d$ and vertices $u,v\in V(G)$ with $d(u,v)=d$ such that \cref{alg:kpr} with adversarial choices of roots in each component and parameter $R > 2d$ never separates $u,v$.
\end{theorem}

\paragraph{Achieving Individual Fairness.} We next show a modification of \cref{alg:kpr} that provides a matching (to within a constant factor) lower bound on the probability of separation when the vertex pairs correspond to edges (that is $d(u,v) = 1$). In other words, any edge $(u,v)$ is cut with probability $\Theta\left(\frac{1}{R}\right)$. This is the algorithm we will implement in our \ldd\ framework.

\gov{Add a name for the algo}
%\subsection{Random Weights}\label{sec:rand-wts}
\begin{algorithm}[htbp]
	\caption{KPR algorithm with random vertex weights}\label{alg:kpr-randwts}
	\hspace*{\algorithmicindent} \textbf{Input}: Integer $R$, planar graph $G=(V,E)$
	\begin{algorithmic}[1]
		\State Set $F\gets \{\}$.
		\For{$i=\{1,2,3\}$}
			\For{every connected component $C$
			of $G\setminus F$}
			\State Perform BFS from an arbitrary root $r$ in $C$.
			\State Sample $\theta$ uniformly at
			random from $\{0,1,\ldots R-1\}$.
			\For{\label{step:forloop}every vertex $v$ at level $\ell_v\equiv \theta \mod R$}
			\State Independently choose $b_v\in \{0,1\}$ uniformly at random.
			\State $\ell_v\gets \ell_v+b_v$
			\EndFor
                \State   For non-negative integers $q$, define $V_q=\{v \mid   q R +\theta < \ell_v \le (q+1)R+\theta\}$. 
			\State Let $E_q$ denote edges with one end-point in set $V_q$, and let $E' = \cup_{q \ge 0} E_q$.
			\State $F\gets F\cup E'$.
			\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}

\begin{theorem}[Proved in \cref{sec:alg-randwts}]
\label{thm:alg-randwts}
\Cref{alg:kpr-randwts} produces components of diameter at most $43 \cdot (R+1)$ and every pair $(u,v) \in V \times V$ satisfies
\begin{align*}
\frac{1}{2R}\leq \Pr[u,v \text{ are separated}]\leq \begin{cases}
3\rho_{uv}+\frac{3}{R} \qquad &\text{ if  $d(u,v)>1$}\\
\frac{3}{R} \qquad &\text{ if  $d(u,v)=1$}\\
\end{cases}.
\end{align*}
\end{theorem}




%For the redistricting application, we choose the diameter $R$ carefully so that each part has population much smaller than the population of a district.  we show that the number of clusters obtained by the decomposition is much smaller than the original number of vertices (precincts). The choice of $R$ also influences Step (2) outlined below. The guarantee we obtain is that for any edge $(u,v) \in E$, the procedure ensures that 
%$$ \frac{1}{10R}  \le \Pr[\mbox{Edge } (u,v) \mbox{ separated}] \le \frac{10}{R}. $$


\subsection{Trade-offs in Individual Fairness Guarantees}
\label{sec:theory-intro}
The randomness in our redistricting scheme comes from the low diameter decompositions, and we therefore seek to study the trade-offs between various desiderata outlined above -- connectivity, compression, and individual fairness -- in depth from a theoretical perspective. In addition to the overall redistricting framework, this theoretical study is one of the main contributions of this paper. 


%In addition to presenting the redistricting framework with provable guarantees and studying its empirical performance, we also consider the theoretical question of fairness in randomized low-diameter decompositions (LDDs), and how it trades off with other desiderata for such decompositions. 

Before presenting our results, we recap the key desiderata from \cref{sec:improve} more formally. Recall the definition of $\rho_{uv} = \frac{d(u,v)}{R}$ from above; this will serve as a benchmark for the probability with which the LDD cuts a pair $(u,v) \in V \times V$. We assume below that any LDD generates clusters of diameter $O(R)$ for given parameter $R$.    %In the description below, we use $\rho_{uv} = \frac{d(u,v)}{R}$ for any $u,v \in V$ as a benchmark for the probability with which the LDD cuts a pair $(u,v) \in V \times V$. Here, $d(u,v)$ is the graph distance.
 
\begin{description}
%\item[(RAD):]  Any cluster has diameter $O(R)$. 
\item[(CON):] Each cluster is a single connected component. 
\item[(COMP):] For a path graph with $n$ vertices, the number of connected clusters created is at most $O\left(\frac{n}{R} \right)$ for any outcome of the randomness. This condition captures that that the LDD compresses a path graph optimally, regardless of the outcome of the randomness.
\item[$(f,g)$-(CUT):] This captures individual fairness. The probability that $(u,v)$ are separated is upper bounded by $f(\rho_{uv})$ and lower bounded by $g(\rho_{uv})$.  In the ideal case as in \cref{eg:grid},  $\Pr[(u,v) \mbox{ is cut}] = \Theta(\rho_{uv})$, so that $f(\rho) = O(\rho)$ and $g(\rho) = \Omega(\rho)$ simultaneously. 
 % This ensures that Step (2) in the framework above is computationally efficient. Though we show empirically that compression happens, this condition is difficult to formally reason about in general planar graphs. We therefore insist that in the simplest case of a line, the compression yields close to the best possible number $\lceil \frac{n}{R} \rceil$ of connected components.
\end{description}

\paragraph{Trade-offs in Desiderata.} Recall that \cref{alg:kpr} satisfies  (CON), $(f,g)$-(CUT) for $f(\rho) = O(\rho)$, and (COMP). However, as we showed in \cref{thm:kpr-negative}, $g(\rho) = 0$ even when $d(u,v) = 1$. 

We next show the following theorem, that extends \cref{thm:alg-randwts} to derive a lower bound on separation probability for non-adjacent vertex pairs.

\begin{theorem}[Proved in \cref{sec:generallb1}]
\label{thm:generallb1}
    There is an algorithm that achieves  (CON), (COMP), $f(\rho) = O(\rho)$, and $g(\rho) = \Omega(\rho^4)$ for any $d(u,v)$.
\end{theorem}

%We show two separate modifications of the KPR procedure that preserve (RAD), (CON), $f(x) \le c \cdot x$ for constant $c$, and $q = \Omega(1)$. The first modification achieves $g(x) = \Omega(x^4)$ for any $d(u,v)$, while the second achieves $g(x) = \Omega(x)$ for $d(u,v) = 1$, hence matching $f(x)$ to constant factors. The latter is the procedure we implement in Step (1) of our framework.

We next show that the above bound on $g$ can be improved if we  violate (COMP).

\begin{theorem}[Proved in \cref{sec:rand-radius}]
\label{thm:generallb2}
For any constant $\eps > 0$, there is an LDD procedure that achieves  (CON), $f(\rho) = O\left(\frac{\rho}{\eps}\right)$, and $g(\rho) = \Omega(\rho^{1+\eps})$. In the limit of $\eps \rightarrow 0$ gives $f(\rho) = O\left(\rho \log \frac{1}{\rho}\right)$ and $g(\rho) = \Omega(\rho)$.
\end{theorem}

We now consider what happens when we are allowed to violate both (CON) and (COMP). Note that \cref{def:ldd} allows for disconnected partitions, as well as for the parameter $R$ to be larger than the diameter of $G$. 

We first show the following theorem:
\begin{theorem}[Proved in \cref{sec:equiv0}]
\label{thm:equiv0}
For any planar graph and parameter $R$, there is an LDD with $f(\rho) = O(\rho)$ and  $g(\rho) = \Omega\left(\frac{\rho}{\sqrt{ \log R}}\right)$.
\end{theorem}

We will next tie the lower bound condition in LDD precisely to the distortion of embedding the graph metric into $\ell_1$. An embedding is a function $h$ that maps the vertices $v$ of $G$ to $s$-dimensional points $h(v)$ (for some $s$) with the guarantee that the $\ell_1$ distance between $h(u)$ and $h(v)$ is at least $d(u,v)$, and at most $\alpha \cdot d(u,v)$. The parameter $\alpha \ge 1$ is termed the {\em distortion}.

\km{If the converse holds only for a specific $R$, it is not very interesting.}

\begin{theorem}[Proved in \cref{sec:equiv}]
\label{thm:equiv}
If there is an LDD procedure for planar graph\footnote{This theorem holds for arbitrary metric spaces and not just shortest path metrics for planar graphs. } $G$ with some parameter $R$ that achieves $f(\rho)/g(\rho) \le \gamma$, then there is an $\ell_1$ embedding of $G$ with distortion $O(\gamma)$. %Conversely, if planar graph $G$ has an $\ell_1$ embedding with distortion $w$, then for any parameter $R$, there is an LDD with $f(\rho)/g(\rho) = O(w)$.
\end{theorem} 

The best known distortion bound for embedding a planar graph into $\ell_1$ is $O(\sqrt{\log n})$, and it is a major open question to improve this to a constant. This implies obtaining the ``optimal bound''  -- $f(\rho) = O(\rho)$ and $g(\rho) = \Omega(\rho)$ simultaneously -- even violating (CON) and (COMP), resolves a major conjecture in metric embeddings, since by the above theorem, this means a constant distortion embedding of $G$ into $\ell_1$. This shows our results for $f(\rho), g(\rho)$ in the previous theorems may be difficult to improve. The tradeoffs above are summarized in \cref{tab:my-table}.

\begin{table}[]
	\centering
	\begin{tabular}{@{}ccccc@{}}
		\toprule
		& CON & COMP & $f(\rho)$ & $g(\rho)$ \\ \midrule
	KPR (\cref{alg:kpr})	& \checkmark    & \checkmark  &  $O(\rho)$ &  $-$ \\ \midrule
	
	\cref{alg:kpr-modified}	& \checkmark    & \checkmark    &  $O(\rho)$ & $\Omega(\rho^4)$  \\ \midrule
	\multirow{2}{*}{\cref{alg:kpr-rand-radius}} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{$-$} &$O\left(\frac{\rho}{\eps}\right)$   & $\Omega(\rho^{1+\epsilon})$, $\eps > 0$  \\ \cmidrule(l){4-5} 
	&               &               &  $O\left(\rho\log \frac{1}{\rho}\right)$     &  $\rho$   \\ \midrule
 	\cref{alg:embed}	& $-$    & $-$   &  $O(\rho)$ & $\Omega\left(\frac{\rho}{\sqrt{\log R}}\right)$ \\
 \bottomrule
	\end{tabular}
	\caption{Tradeoffs in Desiderata.}
	\label{tab:my-table}
\end{table}











==> content/number.tex <==
\section{Proof of \cref{lem:number}}
\label{app:number}


Let $C_1, C_2, C_3$ be the random variables denoting the additional number of components generated in phases $1,2,3$ respectively, and let $C = C_1 + C_2 + C_3$.  Consider the first phase of \cref{alg:kpr} and the associated BFS tree. We can pretend the edges not in the tree don’t exist; this only decreases the number of components generated. Let $a_1, a_2, \ldots, a_q$ denote the number of edges in levels $1, 2, \ldots, q$ in the tree. We pad this sequence with zeros so that the $q$ is a multiple of $R$. We have $\sum_{i=1}^q a_i = n-1 \le n$. If a level $j$ is cut, the number of additional components created is precisely $a_j$. Since any level is chosen for cut with probability $1/R$, we have $\E[C_1] \le n/R$. 

At the end of the first phase, suppose we have components of size $m_1, m_2, \ldots, m_t$. Applying the above argument again to each of these components,  we have $\E[C_2|C_1] \le \sum_{i=1}^t m_i/R \le n/R$, since $ \sum_{i=1}^t m_i \le n$.  A similar argument holds for $\E[C_3]$, completing the proof of the first part by linearity of expectation. 

For the second part, suppose $R = D/\beta$. Then the BFS tree in the first phase has depth at least $D/2$, so that at least $\lfloor \beta/4 \rfloor$ components have diameter at least $R/2$. For each of these components, the BFS tree now has depth at least $R/2$, so at least one component from each has diameter at least $R/4$. Similarly for the third phase, where we obtain a diameter at least $R/8$, completing the proof.

==> content/old_intro.tex <==
Electoral boundary delimitation
is
the general process of drawing the
boundaries of electoral districts \cite{BoundaryDelimitation}.
In the United states,
the process is known as
Electoral redistricting,
and seeks to partition a state into a fixed number of smaller regions, known as districts, each of which elects a representative to the United States Congress or a state legislature.
Though an important aspect of redistricting is to ensure fair representation, it has a long history of controversy and litigation. ``Gerrymandering''
is the process by which a redistricting plan is created to
to favor one political party over another. It refers to the manipulation of district boundaries in a way that
increases the number of districts a party wins in an election.
This practice has a long history a contention issue in American politics, from the 1800s \cite{NPR_2017} to as 
recently as early 2024 \cite{rawstoryDemsPrepare}.

In this paper, we consider the central question of {\em auditing} a given redistricting plan for fairness. Such audit is typically done by randomly sampling redistricting plans and comparing the histogram of the fairness property of interest with the same property for the given plan. Given the centrality of sampling in audit, there are scant approaches to this problem that are both computationally efficient and achieve some provable guarantees on the distribution they sample from. We make progress in this direction via leveraging low diameter graph decompositions (LDDs) in a novel way, leading to a framework with both provable guarantees and good empirical performance. Along the way, we formulate the question of individual fairness in such decompositions, and perform a theoretical study of the trade-offs between individual fairness and other desiderata in these decompositions. 

\gov{Tables 1.1 and 1.2 from \cite{becker2020redistricting}
are quite informative. Should we add something from that
?}

\subsection{Redistricting Desiderata, Audit, and Sampling} 
The input to the redistricting process is typically a planar graph, where the vertices represent precincts of the state and two vertices have an edge between them if the corresponding precincts are adjacent. Given a number of seats $k$, the goal is to find a partition of the graph into $k$ parts called ``districts'', and such a partition is termed a {\em redistricting plan}.

It is commonly agreed~\cite{reynolds_sims,redistricting101} that any redistricting plan should satisfy the following three basic desiderata: The districts have roughly equal population ({\em population balance}); each district should be a connected region ({\em contiguity}); and the districts should not be too ``skinny'' with unnatural shapes ({\em compactness}).  We say that a plan that satisfies population balance and contiguity is {\em feasible}; typically, compactness is considered a measure of fairness and not feasibility. 

\paragraph{Fairness and Audit via Random Sampling.} Beyond these basic desiderata, there is ongoing debate on richer notions of desirability, particularly notions related to the ``fairness'' of a plan, for instance, the seat share it finds for both parties; indeed, compactness has also been considered a fairness property. This has motivated a long line of recent work~\cite{deford2019recombination, deford2020computational, herschlag2017evaluating} as well as software tools~\cite{princeton, redistricting101} on \emph{auditing} a given redistricting plan against various fairness concepts, and such audit tools have been used in arguing and adjudicating legal cases around redistricting~\cite{recomusage,mccartan2022simulated,mattingly2021expert}. 

One popular way to audit a given plan for fairness is via randomly sampling feasible plans~\cite{deford2019recombination, deford2020computational, herschlag2017evaluating}:  First we construct an ensemble of feasible plans by sampling repeatedly from the uniform distribution over all such plans. Then, given an implemented plan, we compare its fairness statistic of interest (such as compactness or seat share) against the corresponding histogram of the same statistic for the ensemble. If the implemented plan is an outlier in this histogram, we can argue it is unfair. Some of these concepts have since been adopted in Wisconsin's and Michigan's redistricting efforts~\cite{recomusage}. 

The challenge with random sampling is that the conditions of feasibility of a plan -- contiguity and balance -- are computationally hard constraints to enforce for any reasonable measure of compactness. Prior work has ruled out existence of computationally efficient and practical schemes that provides samples from the uniform distribution, under natural complexity assumptions. The work of~\cite{najt19sampling} shows that uniformly sampling connected partitions into even two districts is not polynomial time, assuming a standard complexity hypothesis\footnote{The hypothesis they use is $\mathrm{RP}\neq \mathrm{NP}$, which is widely believed to be true.}. Their negative results hold even for a specific class of planar graphs with bounded degree.  We present related complexity results in \cref{sec:related}.

This intractability has motivated heuristic sampling approaches via designing simple Markov chains. The most widely used method, {\sc ReCom}~\cite{deford2019recombination}, defines a chain by merging two adjacent districts, finding a random spanning tree of this merged region, and splitting this tree into two balanced, connected regions. However, there are no guarantees on the distribution such a chain samples from\footnote{Some properties of this chain are known, see for instance~\cite{Charikar-Recom} for  a negative result about mixing time, and~\cite{procaccia2022compact} for a positive result about bias towards compactness.}, and consequently, on the quality of the resulting plans in terms of compactness. 



\subsection{\ldd: Sampling Plans with Guarantees}
In this paper, we propose an alternative framework \ldd\ for generating random feasible redistricting plans. Unlike {\sc ReCom}, the randomness in our procedure does not come from a Markov chain; it instead comes from {\em low diameter decomposition} of the planar graph. In a nutshell, our framework has two steps:

\begin{description}
\item [Low Diameter Decomposition (LDD): ] Given a parameter $R$, the first step partitions the vertices of the graph into disjoint connected components of diameter $O(R)$ in order to match the {\em marginal probability} that a pair of vertices is separated into different components to their graph distance. %In other words, we want to make the probability that vertex pair $(u,v)$ is separated to be comparable to $\rho_{uv} = \frac{d(u,v)}{R}$, where $d(u,v)$ is the graph distance between $u$ and $v$. 
This step randomly {\em compresses} the graph so that connected groups of vertices of small diameter are replaced by ``super-nodes''. The diameter is small enough that each super-node has small population compared to that of a district. Note that this procedure does not produce $k$ clusters, nor does it guarantee population balance. All it achieves is a randomized compression of $G$ into super-nodes.

\item[Redistricting on the Compressed Graph: ] In the second step, we simply solve the redistricting problem on the compressed graph, that is, partition this graph into $k$ connected, compact regions with approximately the same population  in each region (balance condition). Since we partition super-nodes, any upper-bound on the probability of separation of pairs of precincts derived by the LDD is preserved by this step. We use the $k$-median objective in our experiments to achieve compactness. Since each super-node has bounded radius, we can derive a bound on the approximation of the $k$-median objective of our solution to that of the optimal partitioning. We note that our framework is general -- given the compressed graph, we can use other optimization routines in the second step to achieve different notions of compactness and fairness.
\end{description}

Our main focus in this paper is on the first step, since this step injects randomness into the redistricting process. Intuitively, instead of attempting to generate a uniform distribution over all feasible partitions (a computationally hard problem), the LDD attempts to make the probability that vertex pair $(u,v)$ is separated to be comparable to $\rho_{uv} = \frac{d(u,v)}{R}$, where $d(u,v)$ is the graph distance between $u$ and $v$. 

We begin with the classic graph decomposition procedure of Klein, Plotkin, and Rao (KPR)~\cite{KPR} (see \cref{sec:kpr}). This performs an LDD of a planar graph into connected components of diameter $O(R)$ so that the probability of separation of any pair $(u,v)$ is $O(\rho_{uv})$. However, as we show below, this does not quite get us all the way to our goal of matching marginal probabilities.

\paragraph{Individual Fairness in LDD:} For a decomposition procedure to preserve marginal probabilities, it needs to separate pairs $(u,v)$ with probability $\Theta(\rho_{uv})$, so that pairs with comparable distance are separated with comparable probability. We term this {\em individual fairness} due to its connection to a corresponding notion in fair machine learning~\cite{DworkIndividual}.

As our first contribution (\cref{thm:kpr-negative}), we show that the KPR procedure cannot yield an individual fairness guarantee -- for any distance $d$, some pair $(u,v)$ with distance $d(u,v) = d$ is never separated. This means that though the procedure guarantees that the probability that $(u,v)$ is separated is $O(\rho_{uv})$, the actual probability of separation -- zero -- need not be comparable to this quantity.

On the other hand, we present a practical modification of the KPR procedure (\cref{alg:kpr-randwts}) that preserves all properties of the original procedure, and guarantees that any edge $(u,v)$ is separated with probability $\Theta\left(\frac{1}{R}\right)$ (see \cref{thm:alg-randwts}). 

Using this as a starting point, our second contribution is to systematically study the theoretical trade-offs between three desiderata in randomized planar graph partitioning  -- each part in the partition should be a connected component; these components should optimally compress the graph; and the partitioning should be individually fair. We show that in general, obtaining an individual fairness guarantee of $\Theta(\rho_{uv})$ separation probability for each pair $(u,v)$ of vertices resolves a major conjecture in metric embeddings (\cref{thm:generallb2}) and is hence  difficult to resolve. Given this, we show increasingly stronger lower bounds on the separation probability -- that is, achieve stronger individual fairness -- as we relax the requirements; first, with both compression and connectivity (\cref{thm:generallb1}), next relaxing compression (\cref{thm:generallb2}) and finally relaxing connectivity (\cref{thm:equiv0,thm:equiv}).

When run on real data, we show that in this decomposition, each component has population much smaller than that of a single district, yet large enough that the graph is compressed into a smaller collection of super-nodes. We also derive lower and upper bounds for the probability any individual edge $(u,v)$ in the graph is separated by this process, and finally show the effect of incorporating individual fairness.

\paragraph{Balanced $k$-median Clustering.} We next compute the redistricting on the compressed graph. Towards this end, we cluster these super-nodes into $k$ connected regions, each of which is approximately population balanced, while minimizing the $k$-median cost of the clustering. For this, we write the problem as an integer linear program (ILP). The challenge now is computational, since the ILP is too large for integer program solvers. First we consider the LP relaxation and observe that because this is written over a compressed set of nodes afforded by the LDD, it can be solved efficiently.  This LP relaxation yields a lower bound on the $k$-median cost of any balanced clustering of the super-nodes. We then consider the set of centers that are fractionally opened by the LP optimum, and and write the ILP using just these centers. At this point, the ILP with the smaller set of centers and the compressed set of nodes can be efficiently solved. We empirically show that the ILP optimum is close to the LP optimum, and is hence approximately optimum for the overall clustering problem. This yields the final set of districts.

\paragraph{Guarantees and Experiments.} For the choice of parameter $R = ???$, we show two guarantees for the overall process. We note that such guarantees are not obtained by prior sampling approaches. 

\km{Is the above claim correct?}

\begin{description}
    \item[Marginals guarantee:] For any edge $(u,v)$ of the graph $G$, the probability they are separated is at most $???$.
    \item[Compactness guarantee:]  The average $k$-median cost of the final solution is within an additive $2 \hat{R}$ of the $k$-median cost of any balanced redistricting solution, where $\hat{R}$ is the largest diameter of any component in the LDD. We empirically show that $\hat{R} \le ???$.
\end{description}

We perform experiments on ....

\subsection{Related Work}
\label{sec:related}
\paragraph{Redistricting Algorithms.} Modeling redistricting as an optimization problem dates back half a century~\cite{vickrey1961prevention, hess1965nonpartisan} and we refer the reader to~\cite{becker2020redistricting} for a survey. The problem of finding a balanced, contiguous plan that minimizes some measure of compactness is {\sc NP-Hard}~\cite{KoTAM22,kueng19fair,kmeanshard,AwasthiCKS15} under various notions of compactness such as cut edges or $k$-means cost.  Given this intractability, several approaches have been proposed to find the optimum balanced, contiguous, and compact plan. These include the use of Voronoi diagrams~\cite{levin2019automated, gawrychowski2021voronoi,cohen-addad2018balanced}, local search~\cite{king2015efficient}, simulated-annealing~\cite{altman2011bard}, and evolutionary algorithms~\cite{liu2016pear}.

\paragraph{Auditing and Sampling. } Auditing plans for unfairness is widely studied, including in court cases and for state legislatures~\cite{mccartan2022simulated,mattingly2021expert}. Typical fairness properties audited include compactness measures such as Reock~\cite{reock1961note} and Polsby-Popper~\cite{polsby1991third} scores, and electoral outcomes, such as efficiency gap~\cite{stephanopoulos2015partisan}, mean-median gap~\cite{wang2016three}, partisan symmetry~\cite{warrington2018quantifying}, the GEO metric~\cite{campisi2022geography}, and the competitiveness of the plan~\cite{deford2020computational}. Many of these measures are used in publicly available tools~\cite{princeton, GEO}. Other work proposes fairness metrics based on voter stability~\cite{agarwal2021locally}, or methods for ameliorating gerrymandering via multiwinner elections~\cite{garg2021combatting}.

Sampling is a widely implemented method for audit, and was first introduced by Chen and Rodden~\cite{chen2013unintentional}. Other methods for sampling include Flood Fill~\cite{cirincione2000assessing, magleby2018new}, Column Generation~\cite{gurnee2021fairmandering}, and the widely adopted Markov Chain Monte Carlo (MCMC) approach~\cite{tam2016toward, fifield2020automated, lin2022auditing, deford2019recombination, recomusage}. 

On the theoretical front, for the problem of sampling from the uniform distribution, the work of~\cite{cohenaddad21sampling} shows that for graphs with bounded \emph{branch-width}, there is an algorithm that runs in time $O(n^k)$ where $n$ is the number of precincts. They argue that this is close to the best possible in terms of representing the running time with branch-width and $k$. Unfortunately, this result does not translate to a practical algorithm for redistricting, because even simple graphs like the grid have large branch-width relative to $n$. The work of~\cite{procaccia2022compact} shows that the widely used ReCom Markov chain~\cite{deford2019recombination} provably biases towards compact plans.

\paragraph{Low Diameter Decomposition.} Such decomposition of metric spaces are widely used as a subroutine for embedding the metric space into a simpler space such as trees or Euclidean metrics, with provably low distortion, meaning that no distance is stretched too much. We refer the reader to the excellent survey of Matousek~\cite{Matousek2002} for more on such decompositions and their applications. Our application of LDDs is not to embeddings; it is instead to inject randomness to a downstream partitioning problem while making it computationally efficient. As far as we are aware, such an application of LDDs is novel.

==> content/preliminaries.tex <==




==> content/proofs.tex <==
% !TeX root = ./main.tex
%\section{Algorithms}

%We present two different algorithms that modify the Klein, Plotkin, Rao procedure to give lower bounds on the probability of separation. In \Cref{sec:rand-radius}, we present an algorithm that achieves close to the best possible bound possible. Unfortunately, for our experimental evaluations, it produces no usable bound. To this end, we use the algorithm in \Cref{alg:kpr-randwts}. This is the algorithm we will experimentally evaluate for our primary application of redistricting.

\input{lb1}

\input{twocuts}

\input{lb2}

\input{lb3}



\input{equiv}





